Symbolic Verification of Cache Side-channel Freedom

Cache timing attacks allow third-party observers to retrieve sensitive information from program executions. But, is it possible to automatically check the vulnerability of a program against cache timing attacks and then, automatically shield program executions against these attacks? For a given program, a cache configuration and an attack model, our CACHEFIX framework either verifies the cache side-channel freedom of the program or synthesizes a series of patches to ensure cache side-channel freedom during program execution. At the core of our framework is a novel symbolic verification technique based on automated abstraction refinement of cache semantics. The power of such a framework is to allow symbolic reasoning over counterexample traces and to combine it with runtime monitoring for eliminating cache side channels during program execution. Our evaluation with routines from OpenSSL, libfixedtimefixedpoint, GDK and FourQlib libraries reveals that our CACHEFIX approach (dis)proves cache sidechannel freedom within an average of 75 seconds. Besides, in all except one case, CACHEFIX synthesizes all patches within 20 minutes to ensure cache side-channel freedom of the respective routines during execution.

==> acmart-master/Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	sample-manuscript.tex \
	sample-acmsmall.tex \
	sample-acmlarge.tex \
	sample-acmtog.tex \
	sample-sigconf.tex \
	sample-sigconf-authordraft.tex \
	sample-sigplan.tex \
	sample-sigchi.tex \
	sample-sigchi-a.tex


PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf} acmguide.pdf

all:  ${PDF}


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

%.pdf:  %.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

sample-manuscript.pdf \
sample-acmsmall.pdf \
sample-acmlarge.pdf \
sample-acmtog.pdf: samplebody-journals.tex

sample-sigconf.pdf \
sample-sigconf-authordraft.pdf \
sample-sigplan.pdf \
sample-sigchi.pdf: samplebody-conf.tex


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all
	zip $@ acmart.pdf acmguide.pdf sample-*.pdf *.cls *.bst


==> acmart-master/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.  


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
		Sigch-a sample bibliography renamed
		Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
		Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g copyright statements.

==> implementation.tex <==
\section{Implementation and Experimental Setup}
\label{sec:implementation}


==> proof.tex <==
\section{Provable Guarantees}
\label{sec:proof}

We capture an execution trace via a sequence of hits ($h$) and misses ($m$).
% on the alphabet $\{h,m\}$, 
%where $m$ captures a cache miss and $h$ captures a cache hit. 
We model an attacker as the mapping $\objective: \{h,m\}^{*} \rightarrow \mathbb{X}$, 
where $\mathbb{X}$ is a countable set. For ${tr}_1, {tr}_2 \in \{h,m\}^{*}$, an 
attacker can distinguish ${tr}_1$ from ${tr}_2$ if and only if 
$\objective (tr_1) \ne \objective (tr_2)$. In this paper, we instantiate our 
checker for the following two attack models: 
\begin{itemize}
\item $\objective_{time}: \{h,m\}^{*} \rightarrow \mathbb{N}$. 
%The attacker is captured via the mapping 
%$\objective_{time}: \{h,m\}^{*} \rightarrow \mathbb{N}$. In particular, 
$\objective_{time}$ maps each execution trace to the number of cache 
misses suffered by the same. This attack model imitates cache timing 
attacks~\cite{timing-attack-paper}. 

\item $\objective_{trace}: \{h,m\}^{*} \rightarrow \{0,1\}^{*}$. 
%The attacker is modeled via 
%$\objective_{trace}: \{h,m\}^{*} \rightarrow \{0,1\}^{*}$. 
%Concretely, 
$\objective_{trace}$ maps each execution trace to a bitvector 
($h$ is mapped to $0$ and $m$ is mapped to $1$). This attack 
model imitates trace-based attacks~\cite{trace-attack-paper}. 
\end{itemize}

\subsection{Provable guarantees}
\CC satisfies the following crucial properties.
% to guarantee 
%the cache side-channel freedom of a program. 

\begin{app}
\label{prop:monotone}
{\textbf{(Monotonicity)}} 
Consider a victim program $\program$ with sensitive input $\mathcal{K}$. 
Given attack models $\objective_{time}$ or $\objective_{trace}$, assume 
that the channel capacity to quantify the uncertainty of guessing $\mathcal{K}$ 
is $\mathcal{G}_{cap}^{\program}$. Our checker guarantees that $\mathcal{G}_{cap}^{\program}$ 
monotonically decreases with each synthesized patch being applied at runtime. 
\end{app}

\begin{proof}
%We synthesize patches from the counterexample traces generated by our checker. 
%To satisfy the {\em monotonicity property}, we generate counterexamples from 
%our checker in a specific order. To this end, we consider counterexamples that 
%fall into the same equivalence class of observation by the attacker. 
%For instance, in the presence of attacker model $\objective_{time}$, such an 
%equivalence class is based on the total number of cache misses exhibited in a 
%counterexample trace. Intuitively, we explore all counterexamples in the same 
%equivalence class, before moving to explore counterexamples in a different 
%equivalence class. 
%
Consider the generic attack model $\objective: \{h,m\}^{*} \rightarrow \mathbb{X}$ 
that maps each trace to an element in the countable set $\mathbb{X}$. 
For a victim program $\program$, assume $\mathit{TR} \subseteq \{h,m\}^{*}$ is 
the set of all execution traces. After one round of patch synthesis, assume 
$\mathit{TR}' \subseteq \{h,m\}^{*}$ is the set of all execution traces in 
$\program$ when the synthesized patches are applied at runtime. By construction,  
each round of patch synthesis merges two equivalence classes of observations 
({\em cf.} Algorithm~\ref{alg:monitor}), hence, making them indistinguishable 
by the attacker $\objective$. As a result, the following relationship holds:
{%\small
\begin{equation}
\label{eq:trace-neutralize}
\left | \objective (\mathit{TR}) \right | = \left | \objective (\mathit{TR}') \right | + 1
\end{equation} }
Channel capacity $\mathcal{G}_{cap}^{\program}$  equals to 
$\log|\objective (\mathit{TR})|$ for the original 
program $\program$~\cite{dynamic-leakage-paper,qest-paper}, but it reduces to 
$\log|\objective \left ( \mathit{TR}' \right )|$ when the synthesized patches are applied. We conclude 
the proof as the same argument holds for any round of patch synthesis. 
\end{proof}


\begin{app}
\label{prop:converge}
{\textbf{(Convergence)} 
Let us assume a victim program $\program$ with sensitive input $\mathcal{K}$. 
In the absence of any attacker, assume that the uncertainty to guess 
$\mathcal{K}$ is $\mathcal{G}_{cap}^{init}$, $\mathcal{G}_{shn}^{init}$ and 
$\mathcal{G}_{min}^{init}$, via channel capacity, Shannon entropy and Min 
entropy, respectively. If our checker terminates and all synthesized patches 
are applied at runtime, then our framework guarantees that the channel capacity 
(respectively, Shannon entropy and Min entropy) 
will remain $\mathcal{G}_{cap}^{init}$ 
(respectively, $\mathcal{G}_{shn}^{init}$ and $\mathcal{G}_{min}^{init}$) 
even in the presence of attacks captured via $\objective_{time}$ and 
$\objective_{trace}$.}
\end{app}

\begin{proof}
%Consider the generic attack model $\objective: \{h,m\}^{*} \rightarrow \mathbb{X}$, 
%mapping each execution trace to an element in the countable set $\mathbb{X}$. 
%Assume $\program$ exhibits a set of execution traces $\mathit{TR} \subseteq \{h,m\}^{*}$. 
From \autoref{eq:trace-neutralize}, we know that $|\objective (\mathit{TR})|$ 
decreases with each round of patch synthesis, and therefore, $|\objective (\mathit{TR})|$ 
converges to $1$.
%Given that our checker terminates, we obtain the program $\program$, together with 
%a set of synthesized patches that are applied when $\program$ executes. 
If \CC terminates and all patches are synthesized, then assume $\mathit{TR}^{f} \in \{h,m\}^{*}$ 
is the set of execution traces obtained from $\program$ when these patches 
are applied at runtime. 
Clearly, $\left | \objective \left ( \mathit{TR}^{f} \right ) \right | = 1$. 
Therefore, the channel capacity of $\program$, upon the termination of our checker, 
is $\log \left (\left | \objective \left ( \mathit{TR}^{f} \right ) \right | \right )$ = 
$\log 1$ = $0$.

%Given the intuition mentioned in the preceding paragraph, we can now prove the 
%convergence property for our checker. 
%The channel capacity of $\program$, upon the termination of our checker, is 
%$\log \left (\left | \objective \left ( \mathit{TR}^{f} \right ) \right | \right )$ = 
%$\log 1$ = $0$. This concludes that the channel capacity does not change even 
%in the presence of attacks $\objective_{time}$ and $\objective_{trace}$.


For a given distribution $\lambda$ of sensitive input $\mathcal{K}$, Shannon 
entropy $\mathcal{G}_{shn}^{init}$ is computed as follows: 
\begin{equation}
\mathcal{G}_{shn}^{init} (\lambda) = - \sum_{\mathcal{K} \in \mathbb{K}} \lambda(\mathcal{K}) \log_{2} \lambda(\mathcal{K})
\end{equation}
where $\mathbb{K}$ captures the domain of sensitive input $\mathcal{K}$. For 
a given equivalence class of observation $o \in \objective \left ( \mathit{TR}^{f} \right )$, 
the remaining uncertainty is computed as follows: 
\begin{equation}
\label{eq:shannon-remaining-one}
\mathcal{G}_{shn}^{final} (\lambda_o) = - \sum_{\mathcal{K} \in \mathbb{K}} \lambda_o(\mathcal{K}) \log_{2} \lambda_o(\mathcal{K})
\end{equation}
$\lambda_o(\mathcal{K})$ is the probability that the sensitive input is $\mathcal{K}$, 
given the attacker observes $o$. Finally, to evaluate the 
remaining uncertainty of the patched program version, $\mathcal{G}_{shn}^{final} (\lambda_o)$ 
is averaged over all equivalence class of observations as follows:  
\begin{equation}
\label{eq:shannon-remaining-average}
\mathcal{G}_{shn}^{final} \left ( \lambda_{\objective \left ( \mathit{TR}^{f} \right )} \right ) 
= \sum_{o \in \objective \left ( \mathit{TR}^{f} \right )} pr(o)\ \mathcal{G}_{shn}^{final} (\lambda_o)
\end{equation}
$pr(o)$ captures the probability of observation $o \in \objective \left ( \mathit{TR}^{f} \right )$. 
%However, we have $\left | \objective \left ( \mathit{TR}^{f} \right ) \right | = 1$. Hence, for 
%$o \in \objective \left (\mathit{TR}^{f} \right )$, 
We note $pr(o)=1$ and $\lambda_o(\mathcal{K})=\lambda(\mathcal{K})$. 
Plugging these into \autoref{eq:shannon-remaining-average} and \autoref{eq:shannon-remaining-one}, 
we get the following: 
\begin{equation}
\label{eq:proof-shannon}
\boxed{
\begin{split}
\mathcal{G}_{shn}^{final} \left ( \lambda_{\objective \left ( \mathit{TR}^{f} \right ) } \right ) 
&= \sum_{o \in \objective \left ( \mathit{TR}^{f} \right )} \mathcal{G}_{shn}^{final} (\lambda_o) 
\\
&= - \sum_{\mathcal{K} \in \mathbb{K}} \lambda(\mathcal{K}) \log_{2} \lambda(\mathcal{K}) 
= \mathcal{G}_{shn}^{init} (\lambda)
\end{split}}
\end{equation}
Properties on min entropy are derived similarly ({\em cf.} Appendix). 
%Finally, for a given distribution $\lambda$ of sensitive input $\mathcal{K}$, 
%the min entropy $\mathcal{G}_{min}^{init}$ is computed as follows:
%\begin{equation}
%\label{eq:min-entropy}
%\mathcal{G}_{min}^{init} (\lambda) = - \log_{2}\ \max_{\mathcal{K} \in \mathbb{K}}\ \lambda(\mathcal{K}) 
%\end{equation}
%Therefore, min entropy captures the best strategy of an attacker, that is, to 
%choose the most probable secret. 
%
%Similar to Shannon entropy, for a given equivalence class of observation 
%$o \in \objective \left ( \mathit{TR}^{f} \right )$, the remaining 
%uncertainty is computed as follows: 
%\begin{equation}
%\label{eq:min-entropy-observe-one}
%\mathcal{G}_{min}^{init} (\lambda_o) = - \log_{2}\ \max_{\mathcal{K} \in \mathbb{K}}\ \lambda_o(\mathcal{K}) 
%\end{equation}
%$\lambda_o(\mathcal{K})$ captures the probability that the sensitive input is $\mathcal{K}$, 
%given the observation $o$ is made by the attacker.
%
%Finally, we obtain the min entropy of the patched program version via the following 
%relation: 
%{%\small
%\begin{equation}
%\label{eq:minentropy-remaining-average}
%%\begin{split}
%\mathcal{G}_{min}^{final} \left ( \lambda_{\objective \left ( \mathit{TR}^{f} \right ) } \right ) = 
%%\\
%- \log_{2} \sum_{o \in \objective \left ( \mathit{TR}^{f} \right ) } 
%pr(o)\  \max_{\mathcal{K} \in \mathbb{K}}\ \lambda_o(\mathcal{K}) 
%%\end{split}
%\end{equation}}
%
%Since $pr(o)=1$ and $\lambda_o(\mathcal{K})=\lambda(\mathcal{K})$ for any 
%$o \in \objective \left ( \mathit{TR}^{f} \right )$, we get the following from 
%\autoref{eq:minentropy-remaining-average} and \autoref{eq:min-entropy-observe-one}: 
%
%\begin{equation}
%\label{eq:proof-min-entropy}
%\boxed{
%\begin{split}
%\mathcal{G}_{min}^{final}  \left ( \lambda_{\objective \left ( \mathit{TR}^{f} \right ) } \right ) 
%&= - \log_{2} \sum_{o \in \objective \left ( \mathit{TR}^{f} \right )}\ \max_{\mathcal{K} \in \mathbb{K}} 
%\lambda_o(\mathcal{K})
%\\
%&= - \log_{2}\ \max_{\mathcal{K} \in \mathbb{K}}\ \lambda(\mathcal{K}) 
%\\
%&= \mathcal{G}_{min}^{init} (\lambda)
%\end{split}}
%\end{equation}
%\autoref{eq:proof-shannon} and \autoref{eq:proof-min-entropy} conclude this proof. 
%
\end{proof}





==> threat_model.all.tex <==
\section{Threat Model and Provable Guarantees}
\label{sec:threat}

In this section, we will discuss the targeted threat models and the provable 
guarantees provided by our checker. 

\subsection{Threat Model}
%Side-channel attacks are broadly classified into two types: {\em synchronous 
%attack} and {\em asynchronous attack}. In {\em synchronous} attack, an attacker 
%triggers the processing of known inputs, however, such a strategy is 
%impossible for asynchronous attacks. Certainly, synchronous attacks are easier 
%to perform as the attacker does not need to compute the start and end points 
%of the execution of the victim routine. For instance, an attacker can launch 
%a synchronous side-channel attack on an encryption routine by invoking the 
%encryption routine for known plaintext message and by observing the total 
%execution time. Since our work aims to verify the absence of timing channel, 
%we assume the presence of a strong attacker who is capable to launch synchronous 
%side-channel attacks. 
%
We assume that an attacker makes observations on the execution traces of victim 
program $\program$ and the implementation of $\program$ is known to the attacker. 
Besides, there does not exist any {\em error} in the observations made by the 
attacker. We also assume that an attacker can execute arbitrary user-level 
code on the processor that runs the victim program. This, in turn, allows the 
attacker to flush the cache ({\em e.g.} via accessing a large array) before 
the victim routine starts execution. We, however, do not assume that the attacker 
can access the address space of the victim program $\program$. We believe the 
aforementioned assumptions on the attacker are justified, as we aim to verify 
the cache side-channel freedom of programs against {\em strong attacker models}.  

Our checker is most suitable to verify and synthesize countermeasures against 
{\em passive} side-channel attacks. In {\em passive} attacks, an attacker gains 
information from the execution properties ({\em e.g.} timing, cache misses) of 
the victim program ({\em e.g.} timing, cache misses), however, she does not 
tamper ({\em e.g.} modifying cache~\cite{flush-and-reload}) with the execution 
of the victim code. 
%Among others, such tampering 
%may include modifying the cache content while the victim program is in 
%action~\cite{flush-and-reload}. If an attacker can manipulate the execution 
%of the victim program, then we call the respective attacks to be 
%{\em active side-channel attacks}. 
For preventing attacks that tamper with victim program execution, we believe 
additional hardware or firmware support is required. This is to 
restrict permission of executing certain instructions, such as {\em cache flush} 
and {\em cache invalidate}.

We capture an execution trace via a sequence of hits ($h$) and misses ($m$).
% on the alphabet $\{h,m\}$, 
%where $m$ captures a cache miss and $h$ captures a cache hit. 
We model an attacker as the mapping $\objective: \{h,m\}^{*} \rightarrow \mathbb{X}$, where 
$\mathbb{X}$ is a countable set. For ${tr}_1, {tr}_2 \in \{h,m\}^{*}$, an 
attacker can distinguish ${tr}_1$ from ${tr}_2$ if and only if 
$\objective (tr_1) \ne \objective (tr_2)$. In this paper, we instantiate our 
checker for the following two attack models: 
\begin{itemize}
\item $\objective_{time}:$ The attacker is captured via the mapping 
$\objective_{time}: \{h,m\}^{*} \rightarrow \mathbb{N}$. In particular, 
$\objective_{time}$ maps each execution trace to the number of cache 
misses suffered by the same. This attack model imitates cache timing 
attacks~\cite{timing-attack-paper}. 

\item $\objective_{trace}:$ The attacker is modeled via 
$\objective_{trace}: \{h,m\}^{*} \rightarrow \{0,1\}^{*}$. 
Concretely, $\objective_{trace}$ maps each execution trace to a bitvector 
($h$ is mapped to $0$ and $m$ is mapped to $1$). This attack model imitates 
trace-based attacks~\cite{trace-attack-paper}. 
\end{itemize}

\subsection{Provable guarantees}

Our checker satisfies the following crucial properties to guarantee 
the cache side-channel freedom of a program. 

\begin{app}
\label{prop:monotone}
{\textbf{(Monotonicity)}} 
Let us assume a victim program $\program$ with sensitive input $\mathcal{K}$. 
Given attack models $\objective_{time}$ or $\objective_{trace}$, assume 
that the channel capacity to quantify the uncertainty of guessing $\mathcal{K}$ 
is $\mathcal{G}_{cap}^{\program}$. Our checker guarantees that $\mathcal{G}_{cap}^{\program}$ 
monotonically decreases with each synthesized patch being applied at runtime. 
\end{app}

\begin{proof}
We synthesize patches from the counterexample traces generated by our checker. 
To satisfy the {\em monotonicity property}, we generate counterexamples from 
our checker in a specific order. To this end, we consider counterexamples that 
fall into the same equivalence class of observation by the attacker. 
For instance, in the presence of attacker model $\objective_{time}$, such an 
equivalence class is based on the total number of cache misses exhibited in a 
counterexample trace. Intuitively, we explore all counterexamples in the same 
equivalence class, before moving to explore counterexamples in a different 
equivalence class. 

Consider the generic attack model $\objective: \{h,m\}^{*} \rightarrow \mathbb{X}$ 
that maps each trace to an element in the countable set $\mathbb{X}$. 
For a victim program $\program$, assume $\mathit{TR} \subseteq \{h,m\}^{*}$ is 
the set of all execution traces. After one round of patch synthesis, assume 
$\mathit{TR}' \subseteq \{h,m\}^{*}$ is the set of all execution traces in 
$\program$ when the synthesized patches are applied at runtime. By construction,  
each round of patch synthesis merges two equivalence classes of observations, 
hence, making them indistinguishable by the attacker $\objective$. As a result, 
the following relationship holds:
\begin{equation}
\label{eq:trace-neutralize}
\left | \objective (\mathit{TR}) \right | = \left | \objective (\mathit{TR}') \right | + 1
\end{equation} 

Channel capacity $\mathcal{G}_{cap}^{\program}$  equals to 
$\log|\objective (\mathit{TR})|$ for the original 
program $\program$~\cite{dynamic-leakage-paper,qest-paper}, but it reduces to 
$\log|\objective \left ( \mathit{TR}' \right )|$ when the synthesized patches are applied. We conclude 
the proof as the same argument holds for any round of patch synthesis. 

\end{proof}


\begin{app}
\label{prop:converge}
{\textbf{(Convergence)} 
Let us assume a victim program $\program$ with sensitive input $\mathcal{K}$. 
In the absence of any attacker, assume that the uncertainty to guess 
$\mathcal{K}$ is $\mathcal{G}_{cap}^{init}$, $\mathcal{G}_{shn}^{init}$ and 
$\mathcal{G}_{min}^{init}$, via channel capacity, Shannon entropy and Min 
entropy, respectively. If our checker terminates and all synthesized patches 
are applied at runtime, then our framework guarantees that the channel capacity 
(respectively, Shannon entropy and Min entropy) 
will remain $\mathcal{G}_{cap}^{init}$ 
(respectively, $\mathcal{G}_{shn}^{init}$ and $\mathcal{G}_{min}^{init}$) 
even in the presence of attacks captured via $\objective_{time}$ and 
$\objective_{trace}$.}
\end{app}

\begin{proof}
Consider the generic attack model $\objective: \{h,m\}^{*} \rightarrow \mathbb{X}$, 
mapping each execution trace to an element in the countable set $\mathbb{X}$. 
We assume a victim program $\program$ that exhibits a set of execution traces 
$\mathit{TR} \subseteq \{h,m\}^{*}$. 
From \autoref{eq:trace-neutralize}, we know that $|\objective (\mathit{TR})|$ 
decreases with each round of patch synthesis. 
Given that our checker terminates, we obtain the program $\program$, together with 
a set of synthesized patches that are applied when $\program$ executes. 
Assume $\mathit{TR}^{f} \in \{h,m\}^{*}$ is the set of execution traces obtained 
from $\program$ when all patches are systematically applied. 
Clearly, $\left | \objective \left ( \mathit{TR}^{f} \right ) \right | = 1$. 

%Given the intuition mentioned in the preceding paragraph, we can now prove the 
%convergence property for our checker. 
The channel capacity of $\program$, upon the termination of our checker, is 
$\log \left (\left | \objective \left ( \mathit{TR}^{f} \right ) \right | \right )$ = 
$\log 1$ = $0$. This concludes that the channel capacity does not change even 
in the presence of attacks $\objective_{time}$ and $\objective_{trace}$.


For a given distribution $\lambda$ of sensitive input $\mathcal{K}$, Shannon 
entropy $\mathcal{G}_{shn}^{init}$ is computed as follows: 
\begin{equation}
\mathcal{G}_{shn}^{init} (\lambda) = - \sum_{\mathcal{K} \in \mathbb{K}} \lambda(\mathcal{K}) \log_{2} \lambda(\mathcal{K})
\end{equation}
where $\mathbb{K}$ captures the domain of sensitive input $\mathcal{K}$. For 
a given equivalence class of observation $o \in \objective \left ( \mathit{TR}^{f} \right )$, 
the remaining uncertainty is computed as follows: 
\begin{equation}
\label{eq:shannon-remaining-one}
\mathcal{G}_{shn}^{final} (\lambda_o) = - \sum_{\mathcal{K} \in \mathbb{K}} \lambda_o(\mathcal{K}) \log_{2} \lambda_o(\mathcal{K})
\end{equation}
$\lambda_o(\mathcal{K})$ captures the probability that the sensitive input is $\mathcal{K}$, 
given the observation $o$ is made by the attacker. Finally, to evaluate the 
remaining uncertainty of the patched program version, $\mathcal{G}_{shn}^{final} (\lambda_o)$ 
is averaged over all equivalence class of observations as follows:  
\begin{equation}
\label{eq:shannon-remaining-average}
\mathcal{G}_{shn}^{final} \left ( \lambda_{\objective \left ( \mathit{TR}^{f} \right )} \right ) 
= \sum_{o \in \objective \left ( \mathit{TR}^{f} \right )} pr(o)\ \mathcal{G}_{shn}^{final} (\lambda_o)
\end{equation}
where $pr(o)$ captures the probability of the observation $o \in \objective \left ( \mathit{TR}^{f} \right )$. 
However, we have $\left | \objective \left ( \mathit{TR}^{f} \right ) \right | = 1$. Hence, for any 
$o \in \objective \left (\mathit{TR}^{f} \right )$, we get $pr(o)=1$ and $\lambda_o(\mathcal{K})=\lambda(\mathcal{K})$. 
Plugging these observations into \autoref{eq:shannon-remaining-average} and \autoref{eq:shannon-remaining-one}, 
we get the following: 
\begin{equation}
\label{eq:proof-shannon}
\boxed{
\begin{split}
\mathcal{G}_{shn}^{final} \left ( \lambda_{\objective \left ( \mathit{TR}^{f} \right ) } \right ) 
&= \sum_{o \in \objective \left ( \mathit{TR}^{f} \right )} \mathcal{G}_{shn}^{final} (\lambda_o) 
\\
&= - \sum_{\mathcal{K} \in \mathbb{K}} \lambda(\mathcal{K}) \log_{2} \lambda(\mathcal{K}) 
\\
&= \mathcal{G}_{shn}^{init} (\lambda)
\end{split}}
\end{equation}

Finally, for a given distribution $\lambda$ of sensitive input $\mathcal{K}$, 
the min entropy $\mathcal{G}_{min}^{init}$ is computed as follows:
\begin{equation}
\label{eq:min-entropy}
\mathcal{G}_{min}^{init} (\lambda) = - \log_{2}\ \max_{\mathcal{K} \in \mathbb{K}}\ \lambda(\mathcal{K}) 
\end{equation}
Therefore, min entropy captures the best strategy of an attacker, that is, to 
choose the most probable secret. 

Similar to Shannon entropy, for a given equivalence class of observation 
$o \in \objective \left ( \mathit{TR}^{f} \right )$, the remaining 
uncertainty is computed as follows: 
\begin{equation}
\label{eq:min-entropy-observe-one}
\mathcal{G}_{min}^{init} (\lambda_o) = - \log_{2}\ \max_{\mathcal{K} \in \mathbb{K}}\ \lambda_o(\mathcal{K}) 
\end{equation}
$\lambda_o(\mathcal{K})$ captures the probability that the sensitive input is $\mathcal{K}$, 
given the observation $o$ is made by the attacker.

Finally, we obtain the min entropy of the patched program version via the following 
relation: 
{%\small
\begin{equation}
\label{eq:minentropy-remaining-average}
%\begin{split}
\mathcal{G}_{min}^{final} \left ( \lambda_{\objective \left ( \mathit{TR}^{f} \right ) } \right ) = 
%\\
- \log_{2} \sum_{o \in \objective \left ( \mathit{TR}^{f} \right ) } 
pr(o)\  \max_{\mathcal{K} \in \mathbb{K}}\ \lambda_o(\mathcal{K}) 
%\end{split}
\end{equation}}

Since $pr(o)=1$ and $\lambda_o(\mathcal{K})=\lambda(\mathcal{K})$ for any 
$o \in \objective \left ( \mathit{TR}^{f} \right )$, we get the following from 
\autoref{eq:minentropy-remaining-average} and \autoref{eq:min-entropy-observe-one}: 

\begin{equation}
\label{eq:proof-min-entropy}
\boxed{
\begin{split}
\mathcal{G}_{min}^{final}  \left ( \lambda_{\objective \left ( \mathit{TR}^{f} \right ) } \right ) 
&= - \log_{2} \sum_{o \in \objective \left ( \mathit{TR}^{f} \right )}\ \max_{\mathcal{K} \in \mathbb{K}} 
\lambda_o(\mathcal{K})
\\
&= - \log_{2}\ \max_{\mathcal{K} \in \mathbb{K}}\ \lambda(\mathcal{K}) 
\\
&= \mathcal{G}_{min}^{init} (\lambda)
\end{split}}
\end{equation}
\autoref{eq:proof-shannon} and \autoref{eq:proof-min-entropy} conclude this proof. 

\end{proof}




==> threat_model.tex <==
\section{Threat Model}
\label{sec:threat}
%In this section, we discuss the targeted threat models and the provable 
%guarantees provided by our checker. 
%
%\subsection{Threat Model}
%Side-channel attacks are broadly classified into two types: {\em synchronous 
%attack} and {\em asynchronous attack}. In {\em synchronous} attack, an attacker 
%triggers the processing of known inputs, however, such a strategy is 
%impossible for asynchronous attacks. Certainly, synchronous attacks are easier 
%to perform as the attacker does not need to compute the start and end points 
%of the execution of the victim routine. For instance, an attacker can launch 
%a synchronous side-channel attack on an encryption routine by invoking the 
%encryption routine for known plaintext message and by observing the total 
%execution time. Since our work aims to verify the absence of timing channel, 
%we assume the presence of a strong attacker who is capable to launch synchronous 
%side-channel attacks. 
%
We assume that an attacker makes observations on the execution traces of victim 
program $\program$ and the implementation of $\program$ is known to the attacker. 
Besides, there does not exist any {\em error} in the observations made by the 
attacker. We also assume that an attacker can execute arbitrary user-level 
code on the processor that runs the victim program. This, in turn, allows the 
attacker to flush the cache ({\em e.g.} via accessing a large array) before 
the victim routine starts execution. We, however, do not assume that the attacker 
can access the address space of the victim program $\program$. We believe the 
aforementioned assumptions on the attacker are justified, as we aim to verify 
the cache side-channel freedom of programs against {\em strong attacker models}.  

\CC is intended to verify and synthesize countermeasures against 
{\em passive} side-channel attacks. In {\em passive} attacks, an attacker gains 
information from execution properties ({\em e.g.} timing and cache misses) of 
the victim program, however, she does not 
tamper ({\em e.g.} modifying cache~\cite{flush-and-reload}) with the execution 
of the victim code. 
%Among others, such tampering 
%may include modifying the cache content while the victim program is in 
%action~\cite{flush-and-reload}. If an attacker can manipulate the execution 
%of the victim program, then we call the respective attacks to be 
%{\em active side-channel attacks}. 
For such {\em tampering} attacks, we believe 
additional hardware or firmware support is required. This is to 
forbid execution of certain instructions in user mode, e.g., {\em cache-flush} 
and {\em cache-invalidate}.


